3D Point Cloud Reconstruction and SLAM as an Input

To handle the different types of surface reconstruction tasks, we have replicated as well as modified a few of reconstruction methods and have made comparisons between the traditional method and data-driven method for reconstruction the surface of an object with dense point cloud as input. On top of that, we proposed a system using tightly-coupled SLAM as an input to generate deskewed point cloud and odometry and a Truncated Signed Distance Function based Surface Reconstruction Library. To get higher accuracy, IMU(Inertial Measurement Unit) pre-integration and pose graph optimization are conduct in the SLAM part. With the help of the Robot Operating System, we could build a system containing those two parts, which can conduct a real-time outdoor surface reconstruction.

==> image.tex <==
\Figure[t!](topskip=0pt, botskip=0pt, midskip=0pt){interface.png}
{Customization interface using XML.\label{interface}}

\Figure[t!](topskip=0pt, botskip=0pt, midskip=0pt){elasticLidar.png}
{process of Elastic Lidar Fusion.\label{elasticLidar}}

\Figure[t!](topskip=0pt, botskip=0pt, midskip=0pt){surfel.png}
{process of Real-time Scalable Dense Surfel Mapping.\label{surfel}}

\Figure[t!](topskip=0pt, botskip=0pt, midskip=0pt){slam.png}
{process of Efficient Surfel-Based SLAM.\label{slam}}

\Figure[t!](topskip=0pt, botskip=0pt, midskip=0pt){Poisson.png}
{Extracting the iso surface.\label{poisson}}

\Figure[t!](topskip=0pt, botskip=0pt, midskip=0pt){points2surf.png}
{process of points2surf.\label{points2surf}}

